Linear Moment Models to Approximate Knudsen Layers

We propose a well-posed Maxwell-type boundary condition for the linear moment system in half-space. As a reduction of the Boltzmann equation, the moment equations are available to model Knudsen layers near a solid wall, where proper boundary conditions should be prescribed. Utilizing an orthogonal decomposition, we separate the part with a damping term from the system and then impose a new class of Maxwell-type boundary conditions on it. Due to the new boundary condition, we show that the half-space boundary value problem admits a unique solution with explicit expressions. Instantly, the well-posedness of the linear moment system is achieved. We apply the procedure to classical flow problems with the Shakhov collision term, such as the velocity slip and temperature jump problems. The model can capture Knudsen layers with very high accuracy using only a few moments.

==> Makefile <==
JOBNAME=article
LATEX=pdflatex
BIBTEX=bibtex
Texlist=intro HME app kramer temjump numerical

all:
	list='$(Texlist)'; \
	$(LATEX) $(JOBNAME)
	$(BIBTEX) $(JOBNAME)
	$(LATEX) $(JOBNAME)
	$(LATEX) $(JOBNAME)

clean:
	rm $(JOBNAME).aux $(JOBNAME).toc $(JOBNAME).log */*.aux	$(JOBNAME).bbl $(JOBNAME).blg


